The First Quiescent Galaxies in TNG300

We identify the first quiescent galaxies in TNG300, the largest volume of the IllustrisTNG cosmological simulation suite, and explore their quenching processes and time evolution to z=0. We find that the first quiescent galaxies with stellar masses M_* > 3 x 10^{10} M_sun and specific star formation rates sSFR < 10^{-11} yr^{-1} emerge at z~4.2 in TNG300. Suppression of star formation in these galaxies begins with a thermal mode of AGN feedback at z~6, and a kinetic feedback mode acts in each galaxy by z~4.7 to complete the quenching process, which occurs on a time-scale of ~0.35 Gyr. Surprisingly, we find that the majority of these galaxies are not the main progenitors of their z=0 descendants; instead, four of the five galaxies fall into more massive galaxies in subsequent mergers at a range of redshifts 2.5 < z < 0.2. By z=0, these descendants are the centres of galaxy clusters with average stellar masses of 8 x 10^{11} M_sun. We make predictions for the first quenched galaxies to be located by the James Webb Space Telescope (JWST).

==> Makefile <==
BASE_NAME = paper
INPUTS    = $(wildcard *.tex) *.bib

LATEX     = latex
PDFLATEX  = pdflatex
BIBTEX    = bibtex
MAKEINDEX = makeindex

pdf: $(BASE_NAME).pdf
ps: $(BASE_NAME).ps

$(BASE_NAME).pdf: $(BASE_NAME).tex $(INPUTS)
	$(PDFLATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(PDFLATEX) $< 
	$(PDFLATEX) $<

clean:
	rm -f $(BASE_NAME)*.ps $(BASE_NAME)*.dvi *.log \
	      *.aux *.blg *.toc *.brf *.ilg *.ind \
	      missfont.log $(BASE_NAME)*.bbl $(BASE_NAME)*.pdf $(BASE_NAME)*.out \
		  $(BASE_NAME)*.lof $(BASE_NAME)*.lot 

==> tmp.tex <==
\title[The First Quiescent Galaxies in TNG300]{The First Quiescent Galaxies in TNG300}
%\author[E. J. Nelson et al.]{Erica J. Nelson,$^{1,2}$\thanks{E-mail: erica.june.nelson@colorado.edu}}
\author[A. I. Hartley et. al.]{Abigail I. Hartley$^{1}$, %\orcid{0000-0002-5891-1603}
Erica J. Nelson$^{1}$, 
% $^{1}$, 
% Erica J. Nelson %\orcid{0000-0002-7524-374X}
% $^{1}$, 
Katherine A. Suess $^{2,3}$, %\orcid{0000-0002-1714-1905}
Alex M. Garcia$^{4}$ %\orcid{0000-0002-8111-9884 
Minjung Park$^{5}$, %\orcid{0000-0002-8435-9402}
\newline
Rebecca Nevin$^{6}$, %\orcid{0000-0003-1056-8401}
Aimee L. Schechter$^{1}$,  %\orcid{0000-0001-7120-2433}
Sarah Wellons$^{7}$, %\orcid{0000-0002-3977-2724}
Lars Hernquist$^{8}$, 
Annalisa Pillepich$^{9}$,  %\orcid{0000-0003-1065-9274}
\newline
Katherine E. Whitaker $^{10, 11}$, %\orcid{0000-0001-7160-3632} 
Paul Torrey$^{12}$, %\orcid{0000-0002-5653-0786}
Bryan A. Terrazas$^{13}$, %\orcid{0000-0001-5529-7305}
Rachel Bezanson$^{14}$,  %\orcid{0000-0001-5063-8254}
\newline
and Christina C. Williams$^{15,16}$  %\orcid{0000-0003-2919-7495
\\ 
%List of institutions
$^{1}$Department for Astrophysical and Planetary Science, University of Colorado, Boulder, CO 80309, USA\\
$^{2}$Department of Astronomy and Astrophysics, University of California, Santa Cruz, 1156 High Street, Santa Cruz, CA 95064 USA\\
$^{3}$Kavli Institute for Particle Astrophysics and Cosmology and Department of Physics, Stanford University, Stanford, CA 94305, USA\\
$^{4}$Department of Astronomy, University of Florida, 211 Bryant Space Sciences Center, Gainesville, FL 32611, USA\\
$^{5}$Center for Astrophysics $\mid$ Harvard $\&$ Smithsonian, 60 Garden St., Cambridge, MA 02138, USA\\
$^{6}$Fermi National Accelerator Laboratory, Batavia, IL 60510, USA \\
$^{7}$Department of Astronomy, Van Vleck Observatory, Wesleyan University, 96 Foss Hill Drive, Middletown, CT 06459, USA \\
$^{8}$Center for Astrophysics, Harvard University, Cambridge, MA 02138, USA\\
$^{9}$Max-Planck-Institut für Astronomie, K'onigstuhl 17, D-69117 Heidelberg, Germany\\
$^{10}$Department of Astronomy, University of Massachusetts, Amherst, MA 01003, USA\\
$^{11}$Cosmic Dawn Center (DAWN), Denmark\\
$^{12}$ Department of Astronomy, University of Florida, 211 Bryant Space Science Center, Gainesville, FL 32611, USA\\
$^{13}$ Center for Astrophysics, Harvard $\&$ Smithsonian, 60 Garden St., Cambridge, MA, 02138, USA\\
$^{14}$ Department of Physics and Astronomy and PITT PACC, University of Pittsburgh, Pittsburgh, PA 15260, USA\\
$^{15}$ Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721, USA\\
$^{16}$ NSF's National Optical-Infrared Astronomy Research Laboratory, 950 North Cherry Avenue, Tucson, AZ 85719, USA
}

